Do Mature Economies Grow Exponentially?

Most models that try to explain economic growth indicate exponential growth paths. In recent years, however, a lively discussion has emerged considering the validity of this notion. In the empirical literature dealing with drivers of economic growth, the majority of articles is based upon an implicit assumption of exponential growth. Few scholarly articles have addressed this issue so far. In order to shed light on this issue, we estimate autoregressive integrated moving average time series models based on Gross Domestic Product Per Capita data for 18 mature economies from 1960 to 2013. We compare the adequacy of linear and exponential growth models and conduct several robustness checks. Our fndings cast doubts on the widespread belief of exponential growth and suggest a deeper discussion on alternative economic grow theories.

==> latex_sections/chap5_conclusion.tex <==

%This is the Conclusion.
